Emotion Recognition among Couples: A Survey

Couples' relationships affect the physical health and emotional well-being of partners. Automatically recognizing each partner's emotions could give a better understanding of their individual emotional well-being, enable interventions and provide clinical benefits. In the paper, we summarize and synthesize works that have focused on developing and evaluating systems to automatically recognize the emotions of each partner based on couples' interaction or conversation contexts. We identified 28 articles from IEEE, ACM, Web of Science, and Google Scholar that were published between 2010 and 2021. We detail the datasets, features, algorithms, evaluation, and results of each work as well as present main themes. We also discuss current challenges, research gaps and propose future research directions. In summary, most works have used audio data collected from the lab with annotations done by external experts and used supervised machine learning approaches for binary classification of positive and negative affect. Performance results leave room for improvement with significant research gaps such as no recognition using data from daily life. This survey will enable new researchers to get an overview of this field and eventually enable the development of emotion recognition systems to inform interventions to improve the emotional well-being of couples.

==> table_works2.tex <==
% \usepackage{array}
% \usepackage{pdflscape}
% \usepackage{longtable}


\begin{landscape}
\begin{longtable}{|>{\hspace{0pt}}m{0.027\linewidth}|>{\hspace{0pt}}m{0.067\linewidth}|>{\hspace{0pt}}m{0.056\linewidth}|>{\hspace{0pt}}m{0.086\linewidth}|>{\hspace{0pt}}m{0.154\linewidth}|>{\hspace{0pt}}m{0.056\linewidth}|>{\hspace{0pt}}m{0.058\linewidth}|>{\hspace{0pt}}m{0.107\linewidth}|>{\hspace{0pt}}m{0.058\linewidth}|>{\hspace{0pt}}m{0.05\linewidth}|>{\hspace{0pt}}m{0.042\linewidth}|>{\hspace{0pt}}m{0.161\linewidth}|}
\caption{Summary of surveyed works\label{tab:s}}\\ 
\hline
 & \textbf{Reference} & \textbf{Dataset} & \textbf{Modalities} & \textbf{Features } & \textbf{Interpersonal Consideration} & \textbf{Intrapersonal Consideration} & \textbf{Algorithms } & \textbf{Evaluation Approach} & \textbf{Evaluation Metric} & \textbf{Classes} & \textbf{Main Best Results} \endfirsthead 
\hline
1 & Black et al., 2010 \cite{black2010} & UCLA / UW Couples Therapy & Acoustic & 2007 features: 13 functionals over prosodic and spectral low-level descriptors (LLD) & No & No & Linear  SVM, LDA & Leave-one-couple-out cross validation & Accuracy & Binary & - Positive affect: 82\% (female), 75\% (male)- Negative affect: 77\% (female), 76\% (male) \\ 
\hline
2 & Lee et al., 2010 \cite{lee2010} & UCLA / UW Couples Therapy & Acoustic & 14 prosodic features & Yes (Synchrony / Entrainment) & No & Markov models & Leave-one-couple-out cross validation & Accuracy & Binary & Positive vs negative affect: 76\% \\ 
\hline
3 & Lee et al., 2011a \cite{lee2011a} & UCLA / UW Couples Therapy & Acoustic & 13 functionals of prosodic and spectral features & Yes (Synchrony / Entrainment) & No & RBF SVM & Leave-one-couple-out cross validation & Accuracy & Binary & Positive vs negative affect: 51.79\% \\ 
\hline
4 & Lee et al., 2011b \cite{lee2011b} & UCLA / UW Couples Therapy & Acoustic & Prosodic and spectral features & Yes (Synchrony / Entrainment) & Yes (Sailency) & Multiple instance learning (Expectation Maximization Diverse Density) & Leave-one-couple-out cross validation & Accuracy & Binary & Positive vs negative affect: 53.93\% \\ 
\hline
5 & Georgiou et al., 2011 \cite{georgiou2011} & UCLA / UW Couples Therapy & Lexical & Unigram & No & No & Maximum likelihood & Leave-one-couple-out cross validation & Accuracy & Binary & \#SPILL! \\ 
\hline
6 & Gibson et al., 2011 \cite{gibson2011} & UCLA / UW Couples Therapy & Acoustic & 28 features: mean and over 14 spectral (MFCC) features & No & Yes (Sailency) & - RBF SVM as baseline - Diverse Density Support Vector Machine (DD-SVM) & 10-fold cross validation, couple disjoint & Accuracy & Binary & - Positive affect accuracy: 74.3\% (female), 58.6 (male)- Negative affect accuracy: 77.9\% (female), 71.4\% (male)- Sadness: 66.4\% (female), 63.6\% (male) \\ 
\hline
7 & Katsamanis et al., 2011 \cite{katsamanis2011} & UCLA / UW Couples Therapy & Acoustic, LexicalFusion: Unclear & MFCC, TFIDF & No & Yes (Sailency) & - RBF SVM as baseline - Diverse Density Support Vector Machine (DD-SVM). & 10-fold cross validation, couple disjoint & Accuracy & Binary & - Positive affect: 93\% (lexical)- Negative affect: 95\% (lexical)- Sadness: 80\% (lexical) \\ 
\hline
8 & Lee et al., 2012 \cite{lee2012} & UCLA / UW Couples Therapy & Lexical & TFIDF & No & Yes (Sailency) & - Expectation maximization of diverse density function (EM-DD)- Sequential Probability Ratio Test & 10-fold cross validation, couple disjoint & Accuracy & Binary & - Positive affect: 76.1\% - Negative affect: 74.2\% - Sadness: 54.2\% \\ 
\hline
9 & Black et al., 2013 \cite{black2013} & UCLA / UW Couples Therapy & Acoustic & 40,000 and 67,000 features: 14 functionals over prosodic and spectral low-level descriptors (LLD) & No & No &  & Leave-one-couple-out cross validation & Accuracy & Binary & - Positive affect: 77.9\% (female), 72.9 (male)- Negative affect: 80\% (female), 85.7\% (male) \\ 
\hline
10 & Lee et al., 2014 \cite{lee2014} & UCLA / UW Couples Therapy & Acoustic & 35 features. Mean and variance over prosodic and spectral features & Yes (Synchrony / Entrainment) & No &  & Leave-one-couple-out cross validation & Accuracy & Binary & Positive vs negative affect: 62.86\% \\ 
\hline
11 & Chakravarthula et al., 2015 \cite{chakravarthula2015} & UCLA / UW Couples Therapy & Lexical & Unigram & No & Yes (Dynamic modeling) &  & Leave-one-couple-out cross-validation & Accuracy & Binary & Negative affect: 88.57\%(female), 83.57\%(male) \\ 
\hline
12 & Xia el al., 2015 \cite{xia2015} & UCLA / UW Couples Therapy & Acoustic & 6 functionals over prosody and spectral features & No & Yes (Dynamic modeling) &  & Leave-one-couple-out cross-validation & Accuracy & Binary & - Positive affect: 81\% (female), 78 (male)- Negative affect: 79\% (female), 84\% (male)- Sadness: 65\% (female), 61\% (male) \\ 
\hline
13 & Xiao et al., 2015 \cite{xiao2015} & UCLA / UW Couples Therapy & Visual & Line Spectral Frequencies of head motion vectors & Yes (Synchrony / Entrainment) & No & GMM + Linear SVM & Leave-one-couple-out cross-validation & Accuracy & Binary & Positive affect: 63\%Negative affect: 57\% \\ 
\hline
14 & Gibson et al., 2015 \cite{gibson2015} & UCLA / UW Couples Therapy & Acoustic, Lexical, VisualFusion: Feature-level, Decision-level & Acoustic: 90 features. 6 Functionals over 15 LLDs: prosodic (log-pitch, intensity), and spectral (MFCC)Lexical: TFIDFVisual: Power spectral density (PSD) of the head motion vectors & No & Yes (Sailency) & Diverse Density, Linear SVM & Leave-one-couple-out cross-validation & Accuracy & Binary & Positive affect: 65.13\% (all modalities, bag feature-level fusion)Negative affect: 70.34\% (lexical and both feature-level and decision level fusion) \\ 
\hline
15 & Li et al., 2016 \cite{li2016} & UCLA / UW Couples Therapy & Acoustic & 6 functionals over prosodic and spectral features & No & No &  & Leave-one-couple-out cross-validation & Accuracy & Binary & Negative affect: 77.14\% \\ 
\hline
16 & Tseng et al., 2016 \cite{tseng2016} & UCLA / UW Couples Therapy & Lexical & word2vec & No & No &  & Leave-one-couple-out cross-validation & Accuracy & Binary & Negative affect: 88.93\% \\ 
\hline
17 & Tseng et al., 2017 \cite{tseng2017} & UCLA / UW Couples Therapy & Lexical & word2vec, Deep sentence embeddings pretrained using a conversational model which uses seq2seq + attention & No & No & LSTM + RBF SVR & Leave-one-couple-out cross-validation & Mean absolute Error & N/A & Negative affect: 1.37 \\ 
\hline
18 & Li et al., 2017 \cite{li2017} & UCLA / UW Couples Therapy & Acoustic & 420 features: 6 functionals over prosodic and spectral LLD & No & No & DNN (autoencoder) & Leave-one-couple-out cross validation & Accuracy & Binary & Negativity: 69.64\%Positivity: 66.43 \% \\ 
\hline
19 & Chakravarthula et al., 2018 \cite{chakravarthula2018} & UCLA / UW Couples Therapy & Lexical & Ngram & Yes (Dyadic Influence) & Yes (Dynamic modeling) &  & Leave-one-couple-out cross validation & Accuracy & Binary & Negative affect: 88.93\% \\ 
\hline
20 & Tseng et al., 2018 \cite{tseng2018} & UCLA / UW Couples Therapy & Acoustic, LexicalFusion: Feature-level, Decision-level, Gender-based, Therapy Stage & Acoustic: 6 functionals over prosodic and spectral featuresLexical: Deep sentence embeddings pretrained using a conversational model which uses seq2seq + attention & No & No & LSTM, Deep neural network & Leave-one-couple-out cross validation & Mean absolute error & N/A & Negative affect: 1.22 \\ 
\hline
21 & Tseng et al., 2019 \cite{tseng2019} & UCLA / UW Couples Therapy & Lexical & Deep sentence embeddings & No & No & LSTM & Leave-one-couple-out cross validation & Accuracy & Binary & Positivity: 86.8\%Negativity: 87.9\% \\ 
\hline
22 & Chakravarthula et al., 2019 \cite{chakravarthula2019} & Moffit Center Cancer Conversation & Acoustic, LexicalFusion: Feature-level, decision-level & Acoustic: 88 prosodic and spectral eGeMAPS featuresLexical: 600-dimensional deep senstence embedding & No & No & Deep Neural Network & Leave-one-couple-out cross validation & Unweighted Average Recall & 3 & Positive vs Negative vs Neutral: 57.42\% \\ 
\hline
23 & Crangle et al., 2019 \cite{crangle2019} & Stanford Psychotherapy & Acoustic & Prosodic and spectral features & No & No & Random forest & Hold out & Accuracy & 5 & Anger, sadness, joy, tension, neutralCouple A: 87\%(male), 90\%(female)Couple B: 78\%(male), 84\%(female)Couple A: 95\%(male), 88\%(female) \\ 
\hline
24 & Li et al., 2020 \cite{li2020} & UCLA / UW Couples Therapy & Acoustic & 84 features: prosodic and spectral, Deep acoustic embeddings & No & No & CNN, GRU & Leave-4-couples-out cross-validation & Accuracy & Binary & Positivity: 65.36\% Negativity: 76.07\%Sadness: 59.29\% \\ 
\hline
25 & Chakravarthula et al., 2021 \cite{chakravarthula2021} & UCLA / UW Couples Therapy & Lexical & N-gram, ELMo & No & No & Maximum likelihood, GRU & 6-fold cross-validation, couple disjoint & Spearman correlation & N/A & Positive: 0.5 (n-gram), 0.42 (ELMo)Negative: 0.58 (n-gram), 0.52 (ELMo)Anxiety:  0.18 (n-gram), 0.16 (ELMo)Anger: 0.52 (n-gram), 0.50 (ELMo)Sadness: 0.28 (n-gram), 0.34 (ELMo) \\ 
\hline
26 & Boateng et al., 2020 \cite{boateng2020a} & KU Leuven Dyadic Interaction & Acoustic & Spectrograms + Pretrained CNN & No & Yes & Linear SVM & Leave-one-couple-out cross validation & Unweighted Average Recall & Binary & Negative vs Positive valence: 74.8\% (female), 53.3\% (male) \\ 
\hline
27 & Boateng et al., 2021 \cite{boateng2021} & UZH Couples Interaction & Acoustic, LexicalFusion: Feature-level & Acoustic: 172 prosodic and spectral eGeMAPS featuresLexical: Sentence embeddings with Sentence BERT & Yes (Dyadic Influence) & No & Linear SVM, RBF SVM, Random Forest & 10-fold cross validation, couple disjoint & Unweighted Average Recall & Binary & Negative vs Positive valence: 64.8\% (female), 56.1\% (male) \\ 
\hline
28 & Biggiogera et al., 2021 \cite{biggiogera2021} & UZH Couples Interaction & Acoustic, Lexical & Acoustic: 172 prosodic and spectral eGeMAPS featuresLexical: Ngram + TFIDF, LIWC, Sentence embeddings with Sentence BERT & No & No & Linear SVM & 10-fold cross validation, couple disjoint & Unweighted Average Recall & Binary & 2/1/69 \\
\hline
\end{longtable}
\end{landscape}
